SGSH: Stimulate Large Language Models with Skeleton Heuristics for Knowledge Base Question Generation

Knowledge base question generation (KBQG) aims to generate natural language questions from a set of triplet facts extracted from KB. Existing methods have significantly boosted the performance of KBQG via pre-trained language models (PLMs) thanks to the richly endowed semantic knowledge. With the advance of pre-training techniques, large language models (LLMs) (e.g., GPT-3.5) undoubtedly possess much more semantic knowledge. Therefore, how to effectively organize and exploit the abundant knowledge for KBQG becomes the focus of our study. In this work, we propose SGSH--a simple and effective framework to Stimulate GPT-3.5 with Skeleton Heuristics to enhance KBQG. The framework incorporates "skeleton heuristics", which provides more fine-grained guidance associated with each input to stimulate LLMs to generate optimal questions, encompassing essential elements like the question phrase and the auxiliary verb.More specifically, we devise an automatic data construction strategy leveraging ChatGPT to construct a skeleton training dataset, based on which we employ a soft prompting approach to train a BART model dedicated to generating the skeleton associated with each input. Subsequently, skeleton heuristics are encoded into the prompt to incentivize GPT-3.5 to generate desired questions. Extensive experiments demonstrate that SGSH derives the new state-of-the-art performance on the KBQG tasks.

==> ProblemDefine.tex <==
\section{Problem Formulation}
\label{sec:prob}
\begin{figure*}[!t]
\centering 
\includegraphics[width=0.7\textwidth]{AAAI2024/figures/framework.pdf}
\caption{Overview of our SGSH framework, which consists of a PLM-based skeleton generator and a GPT-3.5 model. 
The skeleton generator is trained on the training data, where the target skeletons of the training data are constructed by ours.
Then, the skeleton generator can generate the skeleton of the test instance given a triplets-based sequence with an answer.
Based on the skeleton of the test instance, we retrieve examples similar to it in the training data.
Finally, the skeleton-aware examples and the test sample are fed into GPT-3.5 to generate the final question.}
\label{fig:framework} 
\end{figure*}

KBQG aims to generate the question given a set of triplets with a specific answer.
Let $\mathcal{D} = \{(G_i, a_i, q_i)\}_{i=1}^N$, where 
$G_i$ denotes a subgraph consisting of a set of triplet facts, $a_i$ indicates a certain answer and $q_i$ denotes the target question.
Formally, the objective of KBQG is to learn a mapping function, \emph{i.e.}, $f_{\theta}: (G_{i}, a_i) \xrightarrow[]{} {q}_i$.




==> background.tex <==
\section{Background}
\label{sec:back}
In this section, we aim to answer whether PLMs-based models such as BART~\cite{BART} and T5~\cite{T5} can be directly stimulated to generate high-quality questions. 
In this work, we use BART as the backbone.
We first examine the potential of PLMs-based models to generate excellent questions when stimulated by designed skeletons.
Then, we explore whether open LLMs such as LLaMA~\cite{LLaMA} can outperform PLM-based models.
\subsection{Can we stimulate PLM-based models to generate higher-quality questions?}
\label{subsec:pilot}
From our human experience of analyzing complex English sentences, we first identify the basic grammatical structure and then understand the sentence, which can help us grasp the sentence quickly and accurately.
Inspired by the human cognitive capacity, we use the skeleton (\emph{i.e.}, heart of the sentence) of the target question as a guide to clarify whether BART can be triggered to generate good questions.

\vpara{Modeling.}
We first construct the training data to train BART to generate the skeleton.
\hide{
Then, we concatenate the skeleton with triplets to feed BART to generate the final question.}
Experientially, the core of a question is the interrogative word and its nearby words.
In light of this, we design a simple and effective skeleton.
Based on the built training data, we then train a skeleton generator to obtain skeletons on the test data.
With the skeletons, we append them at the end of the triplets to
encourage BART to generate higher-quality questions.

\vpara{Observation.}
Figure~\ref{fig:example} demonstrates an example. 
Specifically, the skeleton generator (\emph{i.e.}, BART) first generates the skeleton ``\textit{What fantasy film did \_ ?}'' according to the triplets.
And then the skeleton with triplets is fed another BART to guide it to generate superior  questions.
We denote the above approach as BART+Skeleton (abbreviated as B+S).
Alternatively, We denote the method of training BART only on triples as BART.
Figure~\ref{fig:pilot} illustrates the results of BART and B+S in BLEU-1 and ROUGE.
\textcolor{red}{The results show that B+S can generate better questions than vanilla BART, which indicates skeletons play an effective guiding role to stimulate BART on KBQG.}
Since the skeletons contain the prior knowledge about target questions, thus the generation model can learn from them to reduce the learning difficulty.

\vpara{Summary.}
Based on the above observation, we find an intriguing phenomenon that PLM-based models such as BART have decent potential to enhance the performance of KBQG, and the key lies in how to effectively stimulate the model. 
Therefore, we would like to propose a universal learnable framework
that automatically encourages PLM-based models to generate high-quality questions for the KBQG task.
However, as current open LLMs are becoming popular for research, a natural question is raised ``\textit{Are PLMs-based models like BART more effective than open LLMs-based models such as LLaMA}''?
To answer the question, we will elaborate in the next section.


\subsection{Are PLMs-based models more effective than open LLMs-based models?}
\label{subsec:plm_effective}
In this section, we investigate the effectiveness of PLMs-based models such as BART by exploring the performance of BART and open LLMs-based models like LLaMA families (\emph{i.e.},  LLaMA-7B, LLaMA-13B, and LLaMA-33B) on WQ dataset measured by BLEU and ROUGE. 
To answer this question, we conduct preliminary experiments and present the observed results.

\vpara{Modeling.}
For BART, we fully fine-tune it on WQ.
For LLaMA series, we employ the most popular parameter-efficient fine-tuning technique—Low-Rank Adaptation (LORA)\footnote{\href{https://github.com/kuleshov-group/llmtune}{https://github.com/kuleshov-group/llmtune}}~\cite{LORA}, to efficiently fine-tune them on WQ, which is difficult to fully fine-tune due to their billions of parameters and our limited GPU and abundant training data. 

\vpara{Observation.}
Figure~\ref{fig:pilot} illustrates the evaluation results on LLaMA-7B, LLaMA-13B, LLaMA-33B, and BART in BLEU-1 and ROUGE.
We conclude that \textcolor{red}{these LLaMA-based models are consistently inferior to BART}, which represents \textbf{BART is more effective and efficient} because it not only generates better questions but only a small number of parameters (\emph{i.e.}, 140M).
We argue that open LLMs perform well on a variety of tasks, but they may not be the best when compared to small PLMs such as BART on a specific task.
Since LLMs are similar to a generalist in a general field whereas PLMs are more like a specialist in a specific field.

\begin{figure}[!t]
\centering 
\includegraphics[width=0.5\textwidth]{AAAI2024/figures/pilot1.png}
\caption{Results of the pilot study. We fine-tune BART and parameter-efficiently fine-tune the LLaMA family on the WQ dataset and denote these methods as BART, LLaMA-7B, LLaMA-13B, and LLaMA-33B respectively. Additionally, the triplets and the skeleton about the target question are fed to BART, denoting this approach as BART+Skeleton (abbreviated as B+S).
We show the results of these methods as measured by BLEU-1 and ROUGE.
}
\label{fig:pilot} 
\end{figure}

\vpara{Summary.}
In view of these observations, we reveal an interesting phenomenon—PLMs with a small number of parameters have a certain potential to outperform LLMs with a large number of parameters in a specific field.
Additionally, we acknowledge that LLMs possess rich semantic knowledge, so we should make full use of their unique knowledge to help PLMs further improve their performance.
In this paper, we provide a new perspective to exploit LLMs.
Further, we devise a novel framework to take full advantage of the advantages of LLMs and PLMs to boost KBQG.









